Clustering Semantic Predicates in the Open Research Knowledge Graph

When semantically describing knowledge graphs (KGs), users have to make a critical choice of a vocabulary (i.e. predicates and resources). The success of KG building is determined by the convergence of shared vocabularies so that meaning can be established. The typical lifecycle for a new KG construction can be defined as follows: nascent phases of graph construction experience terminology divergence, while later phases of graph construction experience terminology convergence and reuse. In this paper, we describe our approach tailoring two AI-based clustering algorithms for recommending predicates (in RDF statements) about resources in the Open Research Knowledge Graph (ORKG) https://orkg.org/. Such a service to recommend existing predicates to semantify new incoming data of scholarly publications is of paramount importance for fostering terminology convergence in the ORKG. Our experiments show very promising results: a high precision with relatively high recall in linear runtime performance. Furthermore, this work offers novel insights into the predicate groups that automatically accrue loosely as generic semantification patterns for semantification of scholarly knowledge spanning 44 research fields.

==> draft <==
%The evaluation results clearly point out that TF-IDF outperforms the SciBERT vectorization method in all metrics and over all models. That is the model prefers a vectorization over our task-specific data. Note since SciBERT does not have a clustering objective, this model cannot be finetuned for our specific problem. Comparing the models trained on TF-IDF vectors across the clustering algorithms, we see the best performance from K-means in \autoref{table:clustering_evaluation_results} as $0.706$ macro $F1$ at $k=1650$ and $0.655$ micro $F1$ at $k=1850$. And, from \autoref{table:clustering_evaluation_results_agglomerative} agglomerative results show $k=1300$ and $k=2050$ with $0.804$ micro $F1$ and $0.935$ macro $F1$, respectively. Thus, agglomerative clustering method surpasses K-means by nearly 10 points. While macro scores tell us how the system performs overall, the micro scores weighs each test instance equally, i.e. it counts for accurate prediction on predicates level instead of on comparisons level. Based on this, our optimal found model is at $k=1300$ with the highest micro $F1$ using TF-IDF vectorization and agglomerative clustering.


\begin{table}[ht!]
\footnotesize
\centering
\caption{Results of automatically generating contribution predicates groups using K-Means clustering. $K$ was chosen in the range from 200 to 2050 in step sizes of 50. The table shows the most significant results obtained in terms of $P$, $R$, and $F1$.}
    \resizebox{\textwidth}{!}{\begin{tabular}{||c | c | c | c || c | c | c || c | c | c || c | c | c||} 
     \hline 
     - & \multicolumn{6}{c||}{Macro-Average} & \multicolumn{6}{c|}{Micro-Average} \\ [0.5ex] 
     \hline
     - & \multicolumn{3}{c||}{TF-IDF} & \multicolumn{3}{c||}{SciBERT} & \multicolumn{3}{c||}{TF-IDF} & \multicolumn{3}{c||}{SciBERT} \\ 
     \hline
     \thead{Clusters\\$K$} & $P$ & $R$ & $F1$ & $P$ & $R$ & $F1$ & $P$ & $R$ & $F1$ & $P$ & $R$ & $F1$ \\ 
     \hline\hline
    200 & 0.344 & \underline{\textbf{0.957}} & 0.445 & 0.128 & \underline{\textbf{0.678}} & 0.187 & 0.057 & \underline{\textbf{0.953}} & 0.108 & 0.055 & \underline{\textbf{0.634}} & 0.101 \\
    1650 & \underline{\textbf{0.650}} & 0.821 & \underline{\textbf{0.706}} & 0.382 & 0.583 & 0.428 & 0.535 & 0.799 & 0.641 & 0.230 & 0.545 & 0.324 \\
    1850 & 0.649 & 0.779 & 0.694 & 0.417 & 0.585 & 0.458 & \underline{\textbf{0.593}} & 0.732 & \underline{\textbf{0.655}} & 0.272 & 0.548 & 0.364 \\
    2050 & 0.609 & 0.748 & 0.654 & \underline{\textbf{0.447}} & 0.572 & \underline{\textbf{0.479}} & 0.486 & 0.696 & 0.572 & \underline{\textbf{0.319}} & 0.534 & \underline{\textbf{0.399}} \\
    \hline
    \end{tabular}}
\label{table:clustering_evaluation_results}
\end{table}

\begin{table}[ht!]
\footnotesize
\centering
\caption{Results of automatically generating contributions predicates groups using Agglomerative clustering. $K$ was chosen in the range from 200 to 2050 in step sizes of 50. The table shows the most significant results obtained in terms of $P$, $R$, and $F1$.}
    \resizebox{\textwidth}{!}{\begin{tabular}{||c | c | c | c || c | c | c || c | c | c || c | c | c||} 
     \hline 
     - & \multicolumn{6}{c||}{Macro-Average} & \multicolumn{6}{c|}{Micro-Average} \\ [0.5ex] 
     \hline
     - & \multicolumn{3}{c||}{TF-IDF} & \multicolumn{3}{c||}{SciBERT} & \multicolumn{3}{c||}{TF-IDF} & \multicolumn{3}{c||}{SciBERT} \\ 
     \hline
     \thead{Clusters\\$K$} & $P$ & $R$ & $F1$ & $P$ & $R$ & $F1$ & $P$ & $R$ & $F1$ & $P$ & $R$ & $F1$ \\ 
     \hline\hline
    200 & 0.521 & \underline{\textbf{0.970}} & 0.622 & 0.144 & \underline{\textbf{0.705}} & 0.263 & 0.160 & \underline{\textbf{0.979}} & 0.275 & 0.067 & \underline{\textbf{0.676}} & 0.122 \\
    1300 & 0.823 & 0.845 & 0.907 & 0.356 & 0.508 & 0.575 & 0.760 & 0.853 & \underline{\textbf{0.804}} & 0.210 & 0.472 & 0.291 \\
    1450 & 0.837 & 0.822 & 0.914 & 0.371 & 0.478 & 0.603 & 0.782 & 0.807 & 0.794 & 0.225 & 0.440 & \underline{\textbf{0.298}} \\
    2000 & 0.874 & 0.733 & 0.933 & 0.396 & 0.377 & 0.655 & \underline{\textbf{0.835}} & 0.727 & 0.777 & 0.270 & 0.324 & 0.295 \\
    2050 & \underline{\textbf{0.874}} & 0.725 & \underline{\textbf{0.935}} & \underline{\textbf{0.398}} & 0.362 & \underline{\textbf{0.664}} & 0.834 & 0.711 & 0.767 & \underline{\textbf{0.271}} & 0.311 & 0.290 \\
    \hline
    \end{tabular}}
\label{table:clustering_evaluation_results_agglomerative}
\end{table}


\begin{table}[ht!]
\footnotesize
\centering
\caption{ADAPT ME: K-means results with sentence-transformers and special tokens.}
    \resizebox{\textwidth}{!}{\begin{tabular}{||c | c | c | c || c | c | c || c | c | c || c | c | c||} 
     \hline 
     - & \multicolumn{6}{c||}{Macro-Average} & \multicolumn{6}{c|}{Micro-Average} \\ [0.5ex] 
     \hline
     - & \multicolumn{3}{c||}{TF-IDF} & \multicolumn{3}{c||}{SciBERT} & \multicolumn{3}{c||}{TF-IDF} & \multicolumn{3}{c||}{SciBERT} \\ 
     \hline
     \thead{Clusters\\$K$} & $P$ & $R$ & $F1$ & $P$ & $R$ & $F1$ & $P$ & $R$ & $F1$ & $P$ & $R$ & $F1$ \\ 
     \hline\hline
        \hline
        200 & 0.344 & \underline{\textbf{0.957}} & 0.506 & 0.380 & 0.921 & 0.538 & 0.057 & \underline{\textbf{0.953}} & 0.108 & 0.242 & 0.913 & 0.383 \\
        \hline
        250 & 0.384 & 0.917 & 0.541 & 0.417 & 0.918 & 0.574 & 0.075 & 0.926 & 0.138 & 0.281 & 0.903 & 0.428 \\
        \hline
        300 & 0.433 & 0.906 & 0.586 & 0.449 & 0.921 & 0.604 & 0.144 & 0.896 & 0.248 & 0.310 & 0.914 & 0.463 \\
        \hline
        350 & 0.453 & 0.917 & 0.607 & 0.466 & \underline{\textbf{0.924}} & 0.620 & 0.272 & 0.906 & 0.419 & 0.320 & \underline{\textbf{0.919}} & 0.475 \\
        \hline
        400 & 0.472 & 0.902 & 0.619 & 0.474 & 0.909 & 0.623 & 0.237 & 0.909 & 0.377 & 0.320 & 0.888 & 0.470 \\
        \hline
        450 & 0.509 & 0.913 & 0.654 & 0.497 & 0.905 & 0.642 & 0.285 & 0.920 & 0.435 & 0.345 & 0.899 & 0.498 \\
        \hline
        500 & 0.566 & 0.909 & 0.698 & 0.526 & 0.907 & 0.665 & 0.418 & 0.901 & 0.571 & 0.355 & 0.895 & 0.508 \\
        \hline
        550 & 0.541 & 0.901 & 0.676 & 0.534 & 0.900 & 0.670 & 0.345 & 0.897 & 0.498 & 0.402 & 0.888 & 0.554 \\
        \hline
        600 & 0.557 & 0.899 & 0.688 & 0.545 & 0.897 & 0.678 & 0.375 & 0.904 & 0.531 & 0.395 & 0.871 & 0.544 \\
        \hline
        650 & 0.567 & 0.890 & 0.693 & 0.545 & 0.900 & 0.679 & 0.382 & 0.894 & 0.536 & 0.404 & 0.879 & 0.553 \\
        \hline
        700 & 0.572 & 0.882 & 0.694 & 0.561 & 0.894 & 0.690 & 0.379 & 0.885 & 0.531 & 0.405 & 0.876 & 0.554 \\
        \hline
        750 & 0.585 & 0.879 & 0.702 & 0.586 & 0.884 & 0.705 & 0.388 & 0.875 & 0.538 & 0.464 & 0.855 & 0.601 \\
        \hline
        800 & 0.598 & 0.882 & 0.713 & 0.586 & 0.887 & 0.706 & 0.428 & 0.872 & 0.574 & 0.457 & 0.868 & 0.598 \\
        \hline
        850 & 0.605 & 0.884 & 0.719 & 0.602 & 0.887 & 0.717 & 0.424 & 0.886 & 0.573 & 0.465 & 0.884 & 0.609 \\
        \hline
        900 & 0.592 & 0.887 & 0.710 & 0.599 & 0.881 & 0.713 & 0.410 & 0.873 & 0.558 & 0.450 & 0.848 & 0.588 \\
        \hline
        950 & 0.608 & 0.870 & 0.716 & 0.618 & 0.893 & 0.731 & 0.423 & 0.864 & 0.568 & 0.491 & 0.864 & 0.626 \\
        \hline
        1000 & 0.605 & 0.864 & 0.712 & 0.630 & 0.883 & 0.735 & 0.424 & 0.858 & 0.568 & 0.488 & 0.853 & 0.621 \\
        \hline
        1050 & 0.624 & 0.868 & 0.726 & 0.641 & 0.893 & 0.746 & 0.428 & 0.860 & 0.572 & 0.495 & 0.878 & 0.633 \\
        \hline
        1100 & 0.632 & 0.868 & \underline{\textbf{0.731}} & 0.625 & 0.881 & 0.731 & 0.447 & 0.838 & 0.583 & 0.480 & 0.886 & 0.623 \\
        \hline
        1150 & 0.628 & 0.856 & 0.724 & 0.648 & 0.885 & 0.748 & 0.445 & 0.828 & 0.579 & 0.495 & 0.861 & 0.629 \\
        \hline
        1200 & 0.618 & 0.859 & 0.718 & 0.651 & 0.882 & 0.749 & 0.408 & 0.842 & 0.550 & 0.507 & 0.862 & 0.639 \\
        \hline
        1250 & 0.613 & 0.833 & 0.706 & 0.659 & 0.882 & 0.754 & 0.433 & 0.799 & 0.562 & 0.519 & 0.866 & 0.649 \\
        \hline
        1300 & 0.630 & 0.832 & 0.717 & 0.662 & 0.883 & 0.757 & 0.507 & 0.813 & 0.625 & 0.519 & 0.858 & 0.647 \\
        \hline
        1350 & 0.607 & 0.826 & 0.700 & 0.672 & 0.876 & 0.760 & 0.406 & 0.803 & 0.539 & 0.565 & 0.861 & 0.682 \\
        \hline
        1400 & 0.595 & 0.827 & 0.692 & 0.670 & 0.874 & 0.758 & 0.400 & 0.790 & 0.531 & 0.569 & 0.865 & 0.686 \\
        \hline
        1450 & 0.599 & 0.827 & 0.695 & 0.678 & 0.870 & 0.762 & 0.410 & 0.793 & 0.541 & 0.562 & 0.861 & 0.680 \\
        \hline
        1500 & 0.594 & 0.820 & 0.689 & 0.676 & 0.874 & 0.763 & 0.397 & 0.808 & 0.532 & 0.556 & 0.855 & 0.674 \\
        \hline
        1550 & 0.639 & 0.813 & 0.716 & 0.689 & 0.866 & 0.767 & 0.511 & 0.757 & 0.610 & 0.589 & 0.857 & 0.698 \\
        \hline
        1600 & 0.576 & 0.794 & 0.667 & 0.684 & 0.859 & 0.762 & 0.376 & 0.757 & 0.503 & 0.572 & 0.844 & 0.682 \\
        \hline
        1650 & \underline{\textbf{0.650}} & 0.821 & 0.726 & 0.681 & 0.855 & 0.758 & 0.535 & 0.799 & 0.641 & 0.588 & 0.832 & 0.689 \\
        \hline
        1700 & 0.622 & 0.791 & 0.696 & 0.685 & 0.863 & 0.764 & 0.514 & 0.769 & 0.616 & 0.579 & 0.843 & 0.686 \\
        \hline
        1750 & 0.627 & 0.794 & 0.701 & 0.695 & 0.848 & 0.764 & 0.489 & 0.770 & 0.598 & 0.609 & 0.836 & 0.705 \\
        \hline
        1800 & 0.594 & 0.773 & 0.672 & 0.696 & 0.854 & 0.767 & 0.509 & 0.738 & 0.603 & 0.607 & 0.848 & 0.707 \\
        \hline
        1850 & 0.649 & 0.779 & 0.708 & 0.704 & 0.849 & 0.770 & \underline{\textbf{0.593}} & 0.732 & \underline{\textbf{0.655}} & 0.603 & 0.834 & 0.700 \\
        \hline
        1900 & 0.632 & 0.773 & 0.695 & 0.707 & 0.838 & 0.767 & 0.564 & 0.723 & 0.634 & 0.614 & 0.818 & 0.702 \\
        \hline
        1950 & 0.628 & 0.763 & 0.689 & 0.712 & 0.842 & 0.771 & 0.584 & 0.713 & 0.642 & 0.620 & 0.834 & 0.711 \\
        \hline
        2000 & 0.624 & 0.750 & 0.682 & 0.725 & 0.843 & 0.779 & 0.552 & 0.699 & 0.617 & 0.659 & 0.813 & 0.728 \\
        \hline
        2050 & 0.609 & 0.748 & 0.672 & \underline{\textbf{0.728}} & 0.844 & \underline{\textbf{0.781}} & 0.486 & 0.696 & 0.572 & \underline{\textbf{0.659}} & 0.808 & \underline{\textbf{0.726}} \\
        \hline
    \end{tabular}}
\label{table:clustering_evaluation_results_k_means}
\end{table}

\begin{table}[ht!]
\footnotesize
\centering
\caption{ADAPT ME: Agglomerative results with sentence-transformers and special tokens.}
    \resizebox{\textwidth}{!}{\begin{tabular}{||c | c | c | c || c | c | c || c | c | c || c | c | c||} 
     \hline 
     - & \multicolumn{6}{c||}{Macro-Average} & \multicolumn{6}{c|}{Micro-Average} \\ [0.5ex] 
     \hline
     - & \multicolumn{3}{c||}{TF-IDF} & \multicolumn{3}{c||}{SciBERT} & \multicolumn{3}{c||}{TF-IDF} & \multicolumn{3}{c||}{SciBERT} \\ 
     \hline
     \thead{Clusters\\$K$} & $P$ & $R$ & $F1$ & $P$ & $R$ & $F1$ & $P$ & $R$ & $F1$ & $P$ & $R$ & $F1$ \\ 
     \hline\hline
        \hline
        200 & 0.521 & \underline{\textbf{0.970}} & 0.678 & 0.309 & 0.031 & 0.056 & 0.160 & \underline{\textbf{0.979}} & 0.275 & 0.198 & 0.032 & 0.055 \\
        \hline
        250 & 0.550 & 0.967 & 0.701 & 0.354 & \underline{\textbf{0.031}} & \underline{\textbf{0.057}} & 0.189 & 0.977 & 0.317 & 0.265 & 0.032 & 0.057 \\
        \hline
        300 & 0.575 & 0.961 & 0.720 & 0.369 & 0.031 & 0.057 & 0.210 & 0.970 & 0.346 & 0.293 & 0.032 & 0.058 \\
        \hline
        350 & 0.592 & 0.955 & 0.731 & 0.390 & 0.030 & 0.056 & 0.239 & 0.964 & 0.383 & 0.312 & \underline{\textbf{0.032}} & \underline{\textbf{0.058}} \\
        \hline
        400 & 0.628 & 0.954 & 0.757 & 0.441 & 0.028 & 0.053 & 0.271 & 0.963 & 0.424 & 0.376 & 0.030 & 0.055 \\
        \hline
        450 & 0.648 & 0.948 & 0.770 & 0.479 & 0.027 & 0.051 & 0.296 & 0.956 & 0.451 & 0.420 & 0.029 & 0.055 \\
        \hline
        500 & 0.676 & 0.945 & 0.788 & 0.494 & 0.026 & 0.050 & 0.365 & 0.954 & 0.528 & 0.425 & 0.027 & 0.051 \\
        \hline
        550 & 0.694 & 0.938 & 0.798 & 0.499 & 0.026 & 0.050 & 0.428 & 0.946 & 0.589 & 0.435 & 0.027 & 0.051 \\
        \hline
        600 & 0.706 & 0.931 & 0.803 & 0.499 & 0.026 & 0.050 & 0.451 & 0.940 & 0.609 & 0.435 & 0.027 & 0.051 \\
        \hline
        650 & 0.724 & 0.927 & 0.813 & 0.499 & 0.026 & 0.050 & 0.468 & 0.937 & 0.624 & 0.435 & 0.027 & 0.051 \\
        \hline
        700 & 0.740 & 0.921 & 0.821 & 0.482 & 0.025 & 0.047 & 0.529 & 0.931 & 0.675 & 0.414 & 0.025 & 0.046 \\
        \hline
        750 & 0.758 & 0.915 & 0.829 & 0.530 & 0.024 & 0.046 & 0.554 & 0.926 & 0.693 & 0.515 & 0.024 & 0.046 \\
        \hline
        800 & 0.768 & 0.907 & 0.832 & 0.530 & 0.024 & 0.046 & 0.576 & 0.918 & 0.708 & 0.522 & 0.024 & 0.046 \\
        \hline
        850 & 0.777 & 0.904 & 0.835 & 0.557 & 0.024 & 0.046 & 0.610 & 0.915 & 0.732 & 0.547 & 0.024 & 0.046 \\
        \hline
        900 & 0.781 & 0.895 & 0.834 & 0.569 & 0.024 & 0.046 & 0.623 & 0.905 & 0.738 & 0.562 & 0.024 & 0.047 \\
        \hline
        950 & 0.790 & 0.885 & 0.835 & 0.617 & 0.023 & 0.043 & 0.665 & 0.890 & 0.761 & 0.646 & 0.024 & 0.046 \\
        \hline
        1000 & 0.799 & 0.881 & 0.838 & 0.617 & 0.023 & 0.043 & 0.696 & 0.886 & 0.780 & 0.646 & 0.024 & 0.046 \\
        \hline
        1050 & 0.805 & 0.873 & 0.838 & 0.606 & 0.022 & 0.042 & 0.727 & 0.879 & 0.796 & 0.639 & 0.023 & 0.044 \\
        \hline
        1100 & 0.811 & 0.869 & \underline{\textbf{0.839}} & 0.621 & 0.022 & 0.042 & 0.736 & 0.875 & 0.799 & 0.648 & 0.023 & 0.045 \\
        \hline
        1150 & 0.813 & 0.866 & 0.839 & 0.635 & 0.021 & 0.041 & 0.742 & 0.872 & 0.802 & 0.668 & 0.023 & 0.044 \\
        \hline
        1200 & 0.817 & 0.859 & 0.838 & 0.706 & 0.021 & 0.041 & 0.746 & 0.865 & 0.801 & 0.721 & 0.023 & 0.044 \\
        \hline
        1250 & 0.819 & 0.851 & 0.835 & 0.728 & 0.021 & 0.041 & 0.751 & 0.859 & 0.801 & 0.752 & 0.023 & 0.044 \\
        \hline
        1300 & 0.823 & 0.845 & 0.834 & 0.751 & 0.021 & 0.041 & 0.760 & 0.853 & \underline{\textbf{0.804}} & 0.761 & 0.023 & 0.044 \\
        \hline
        1350 & 0.828 & 0.839 & 0.834 & 0.762 & 0.020 & 0.040 & 0.769 & 0.826 & 0.796 & 0.787 & 0.022 & 0.043 \\
        \hline
        1400 & 0.831 & 0.831 & 0.831 & 0.759 & 0.020 & 0.038 & 0.772 & 0.819 & 0.795 & 0.772 & 0.019 & 0.036 \\
        \hline
        1450 & 0.837 & 0.822 & 0.829 & 0.764 & 0.020 & 0.038 & 0.782 & 0.807 & 0.794 & 0.776 & 0.019 & 0.036 \\
        \hline
        1500 & 0.838 & 0.813 & 0.825 & 0.755 & 0.019 & 0.037 & 0.783 & 0.799 & 0.791 & 0.769 & 0.018 & 0.035 \\
        \hline
        1550 & 0.841 & 0.810 & 0.825 & 0.755 & 0.019 & 0.037 & 0.789 & 0.796 & 0.793 & 0.769 & 0.018 & 0.035 \\
        \hline
        1600 & 0.845 & 0.800 & 0.822 & 0.783 & 0.019 & 0.037 & 0.799 & 0.789 & 0.794 & 0.781 & 0.018 & 0.035 \\
        \hline
        1650 & 0.848 & 0.796 & 0.821 & 0.783 & 0.019 & 0.037 & 0.808 & 0.778 & 0.792 & 0.781 & 0.018 & 0.035 \\
        \hline
        1700 & 0.853 & 0.784 & 0.817 & 0.762 & 0.017 & 0.033 & 0.813 & 0.768 & 0.790 & 0.760 & 0.016 & 0.031 \\
        \hline
        1750 & 0.857 & 0.779 & 0.816 & 0.760 & 0.016 & 0.031 & 0.818 & 0.764 & 0.790 & 0.758 & 0.015 & 0.029 \\
        \hline
        1800 & 0.857 & 0.770 & 0.812 & 0.792 & 0.014 & 0.028 & 0.819 & 0.758 & 0.787 & 0.809 & 0.013 & 0.026 \\
        \hline
        1850 & 0.862 & 0.765 & 0.810 & 0.792 & 0.014 & 0.028 & 0.824 & 0.752 & 0.787 & 0.809 & 0.013 & 0.026 \\
        \hline
        1900 & 0.865 & 0.759 & 0.808 & 0.782 & 0.013 & 0.026 & 0.827 & 0.747 & 0.785 & 0.796 & 0.012 & 0.024 \\
        \hline
        1950 & 0.869 & 0.743 & 0.801 & \underline{\textbf{0.823}} & 0.013 & 0.026 & 0.830 & 0.735 & 0.779 & \underline{\textbf{0.828}} & 0.012 & 0.024 \\
        \hline
        2000 & \underline{\textbf{0.874}} & 0.733 & 0.797 & 0.823 & 0.013 & 0.026 & \underline{\textbf{0.835}} & 0.727 & 0.777 & 0.828 & 0.012 & 0.024 \\
        \hline
        2050 & 0.874 & 0.725 & 0.793 & 0.823 & 0.013 & 0.026 & 0.834 & 0.711 & 0.767 & 0.828 & 0.012 & 0.024 \\
        \hline

    \end{tabular}}
\label{table:clustering_evaluation_results_agglomerative}
\end{table}
